ArrowGAN : Learning to Generate Videos by Learning Arrow of Time

Training GANs on videos is even more sophisticated than on images because videos have a distinguished dimension: time. While recent methods designed a dedicated architecture considering time, generated videos are still far from indistinguishable from real videos. In this paper, we introduce ArrowGAN framework, where the discriminators learns to classify arrow of time as an auxiliary task and the generators tries to synthesize forward-running videos. We argue that the auxiliary task should be carefully chosen regarding the target domain. In addition, we explore categorical ArrowGAN with recent techniques in conditional image generation upon ArrowGAN framework, achieving the state-of-the-art performance on categorical video generation. Our extensive experiments validate the effectiveness of arrow of time as a self-supervisory task, and demonstrate that all our components of categorical ArrowGAN lead to the improvement regarding video inception score and Frechet video distance on three datasets: Weizmann, UCFsports, and UCF-101.

==> tables/Categorical_all.tex <==
\begin{table*}[t]
  \centering\resizebox{.99\textwidth}{!}{
  \begin{tabular}{l|ccc|cccc}
    \cline{1-8}\cline{1-8}
    \multirow{2}{*}{Baseline}&\multicolumn{3}{c}{Methods} & \multicolumn{2}{c}{\textit{Weizmann}} & \multicolumn{2}{c}{\textit{UCF-101}} \\ \cline{2-8}
    & \begin{tabular}[c]{@{}c@{}}Self\\ Supervised\end{tabular}& Projection & \begin{tabular}[c]{@{}c@{}}Mode\\ Seeking
  \end{tabular}  & IS($\uparrow$) & FID($\downarrow$) & IS($\uparrow$) & FID($\downarrow$) \\
  \hline\hline
 \multicolumn{1}{l|}{conditional TGAN~\cite{saito2017temporal}} & & &   & - & - & 15.83$\pm$.18& -\\\hline
 \multicolumn{1}{l|}{categorical MoCoGAN~\cite{tulyakov2018mocogan}} & & & & 3.16$\pm$.02&3296& 12.29$\pm$.08& 74297\\\hline
\multirow{3}{*}{ours}&$\checkmark$&  & &2.81$\pm$.00& 1022 & 17.34$\pm$.10& 68462\\
& $\checkmark$&$\checkmark$ &  & 3.50$\pm$.02 & 597 & 16.93$\pm$.16 &80002\\
& $\checkmark$& $\checkmark$ & $\checkmark_{AoT}$& \textbf{3.54}$\pm$\textbf{.06}& \textbf{568} & \textbf{18.88}$\pm$\textbf{.08}&\textbf{65762} \\ %epoch 37
\cline{1-8}\cline{1-8} 
\end{tabular}}
\vspace{3mm}
\caption{Effectiveness of components to build the categorical ArrowGAN. Each components shows the improvement of generating videos progressively by IS and FID scores.}
\label{tab:ablation all}
\end{table*}

==> tables/Categorical_all_v2.tex <==
\begin{table*}[t]
\caption{Effectiveness of components to build the categorical ArrowGAN. Each components shows the improvement of generating videos progressively by IS and FID scores. \kb{여기에 설명을 적어주는게 더 괜찮을 것 같습니다. 첫번째 row는 categorical MoCoGAN~\cite{tulyakov2018mocogan}}이며, 각각 어떻게 module을 더했고 그에 따라 Datset별로 어떤 성능 향상이 있었는지}
  \centering\resizebox{.97\textwidth}{!}{
  \begin{tabular}{ccc|cc|cc}
    \cline{1-7}\cline{1-7}
    \multicolumn{3}{c|}{Methods} & \multicolumn{2}{c|}{\textit{Weizmann}} & \multicolumn{2}{c}{\textit{UCF-101}} \\ \cline{1-7}
    ~~~\begin{tabular}[c]{@{}c@{}}Self\\Supervised\end{tabular}~~~& Projection &~~~\begin{tabular}[c]{@{}c@{}}Mode\\Seeking
  \end{tabular}~~~& IS($\uparrow$) &~~~FVD($\downarrow$)~~~& IS($\uparrow$) &~~~FVD($\downarrow$)~~~\\
  \hline\hline
  & & &~~4.41$\pm$.01~~~& 30.69$\pm$.06 &~~12.32$\pm$.14~~~&41.06$\pm$.05 \\\hline
$\checkmark_{AoT}$&  & & 4.72$\pm$.03 & 24.06$\pm$.05 &  & \\
$\checkmark_{AoT}$&$\checkmark$ &  & 4.98$\pm$.02 & 20.41$\pm$.03 & 23.53$\pm$.15&28.56$\pm$.13 \\ %23.64$\pm$.26 & \\
$\checkmark_{AoT}$& $\checkmark$ & $\checkmark$& \textbf{5.35}$\pm$.03& \textbf{15.87}$\pm$.03 & \textbf{26.80}$\pm$.11& \textbf{27.82}$\pm$.13 \\
\hline \hline
\multicolumn{3}{c|}{Real dataset} & \multicolumn{1}{c}{5.64} & \multicolumn{1}{c|}{6.02} & \multicolumn{1}{c}{34.55} & 0.68 \\
\cline{1-7}\cline{1-7} 
\end{tabular}
}
%\vspace{3mm}
\label{tab:ablation all}
\end{table*}

==> tables/Categorical_all_v3.tex <==
\begin{table*}[t]
\caption{Effectiveness of components to build the categorical ArrowGAN. Each components shows the improvement of generating videos progressively by IS and FID scores. \kb{여기에 설명을 적어주는게 더 괜찮을 것 같습니다. 첫번째 row는 categorical MoCoGAN~\cite{tulyakov2018mocogan}}이며, 각각 어떻게 module을 더했고 그에 따라 Datset별로 어떤 성능 향상이 있었는지}
  \centering\resizebox{.97\textwidth}{!}{
  \begin{tabular}{ccc|cc|cc}
    \cline{1-7}\cline{1-7}
    \multicolumn{3}{c|}{Methods} & \multicolumn{2}{c|}{\textit{Weizmann}} & \multicolumn{2}{c}{\textit{UCF-101}} \\ \cline{1-7}
    ~~~projection~~~& \begin{tabular}[c]{@{}c@{}}AoT\end{tabular} &~~~\begin{tabular}[c]{@{}c@{}}diversity\\sensitive
  \end{tabular}~~~& IS($\uparrow$) &~~~FVD($\downarrow$)~~~& IS($\uparrow$) &~~~FVD($\downarrow$)~~~\\
  \hline\hline
            &                   &               &~~~4.41$\pm$.01~~~     & 30.69$\pm$.06 &~~12.32$\pm$.14~~~& 41.06$\pm$.05 \\\hline
$\checkmark$&                   &               & 4.86$\pm$.01         & 21.62$\pm$.05 & 22.60$\pm$.23    & 27.27$\pm$.06\\
$\checkmark$&$\checkmark_{AoT}$ &               & 4.98$\pm$.02         & 20.41$\pm$.03 & 23.53$\pm$.15    & 28.56$\pm$.13 \\
$\checkmark$& $\checkmark_{AoT}$ & $\checkmark$& \textbf{5.35}$\pm$.03 & \textbf{15.87}$\pm$.03 & \textbf{26.80}$\pm$.11 & \textbf{27.82}$\pm$.13 \\
\hline \hline
\multicolumn{3}{c|}{Real dataset} & \multicolumn{1}{c}{5.64} & \multicolumn{1}{c|}{6.02} & \multicolumn{1}{c}{34.55} & 0.68 \\
\cline{1-7}\cline{1-7} 
\end{tabular}
}
%\vspace{3mm}
\label{tab:ablation all}
\end{table*}

==> tables/Uncond_UCF101.tex <==
\begin{table*}[h]
\centering
\resizebox{.80\textwidth}{!}{
\smallskip\begin{tabular}{c|c|cc|cc}
    \cline{1-6}\cline{1-6}
     & \multicolumn{1}{c|}{\textit{UCF-101}} & \multicolumn{2}{c|}{\textit{Weizmann}}& \multicolumn{2}{c}{\textit{UCFsports}}  \\ \cline{2-6}
    Method & IS($\uparrow$)  & IS($\uparrow$) & FID($\downarrow$) & IS($\uparrow$) & FID($\downarrow$)\\
    \hline\hline
    {VGAN} & 9.27$\pm$.03 / 8.18 $\pm$$.05^{\dagger}$  & 2.62$\pm$.02 & 485 & 1.22$\pm$.00 & 5218\\ 
    {TGAN} & 11.17$\pm$.02 / 11.85$\pm$$.07^{\dagger}$  & 3.59$\pm$.01 & 524 & 2.39$\pm$.02 & 3880 \\ 
    {MoCoGAN} & 10.25$\pm$.05 / 12.42$\pm$$.03^{\dagger}$ & 4.25$\pm$.01 & 493 & 2.74$\pm$.01 & 3626\\  \cline{1-6}
    {Arrow-VGAN} & 10.47$\pm$.14 & 3.33$\pm$.01 & 605 & 2.49$\pm$.01 & 4931 \\
    {Arrow-TGAN} & 12.51$\pm$.06 & 4.32$\pm$.02 & 467 & 2.81$\pm$.23 & 3880 \\
    {Arrow-MoCoGAN} & 11.18$\pm$.03  & 4.41$\pm$.01 & 463 & 2.76$\pm$.01 & 3711 \\
    \cline{1-6}
    {Real dataset} & 34.49 & 5.66 & 0.008 & 7.29 & 0.014 \\
    \cline{1-6}\cline{1-6}
  \end{tabular}
}
\vspace{3mm}
\caption{Effectiveness of adding ArrowGAN on baselines. It improves all three baselines in UCF-101. $\dagger$ notices that IS values are taken from MoCoGAN~\cite{tulyakov2018mocogan}, and other values are taken from our reproduced models.}
\label{tab:Uncond UCF101}
\end{table*}

==> tables/ablation_all.tex <==
\begin{table*}[t]
  \centering\resizebox{.75\textwidth}{!}{
  \begin{tabular}{ccc|cccc}
    \cline{1-7}\cline{1-7}
    \multicolumn{3}{c}{Method} & \multicolumn{2}{c}{\textit{Weizmann}} & \multicolumn{2}{c}{\textit{UCF-101}} \\ \cline{1-7}
    Projection & \begin{tabular}[c]{@{}c@{}}Mode\\ Seeking
  \end{tabular} & \begin{tabular}[c]{@{}c@{}}Self\\ Supervised\end{tabular} & IS($\uparrow$) & FID($\downarrow$) & IS($\uparrow$) & FID($\downarrow$) \\
  \hline\hline
 & & &3.16$\pm$.02&3296& 12.29$\pm$.08& 74297\\
\cline{1-7}
$\checkmark$&  & &2.81$\pm$.00& 1022 & 17.34$\pm$.10& 68462\\
%$\checkmark$&  $\checkmark_{AoT}$& & 3.34$\pm$.02 & \textbf{558} & 17.22$\pm$.04&68944\\
$\checkmark$&$\checkmark$ &  & 3.50$\pm$.02 & 597 & 16.93$\pm$.16 &80002\\
$\checkmark$& $\checkmark$ & $\checkmark_{AoT}$& \textbf{3.54}$\pm$\textbf{.06}& \textbf{568} & \textbf{18.88}$\pm$\textbf{.08}&\textbf{65762} \\ %epoch 37
\cline{1-7}\cline{1-7} 
\end{tabular}}
\vspace{3mm}
\caption{Effectiveness of components to build the categorical ArrowGAN. Each components shows the improvement of generating videos progressively by IS and FID scores.}
\label{tab:ablation all}
\end{table*}

==> tables/ablation_temporal.tex <==

\begin{table}[h]
\centering
\begin{tabular}{ccc|c|c|c|c}
\cline{1-7}\cline{1-7}
\multicolumn{3}{c|}{Methods} & \multicolumn{2}{c|}{Weizmann} & \multicolumn{2}{c}{UCFsports} \\ \hline
\multicolumn{1}{c}{AoT} &
\multicolumn{1}{c}{\begin{tabular}[c|]{@{}c@{}}Rotation of \\video\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Rotation of \\frame\end{tabular}} & \multicolumn{1}{c|}{IS($\uparrow$)} & \multicolumn{1}{c|}{FID($\downarrow$)} & \multicolumn{1}{c|}{IS($\uparrow$)} & \multicolumn{1}{c}{FID($\downarrow$)} \\ \hline
\hline
 &  &  & 2.827 & 680 & 2.077 & 3765 \\
 & \checkmark &            & 3.124 & 614 & 2.129 & 3769 \\
 & \checkmark & \checkmark & 1.776 & 712 & 1.628 & 4022 \\
\checkmark &  & \checkmark & 2.615 & 575 & 2.008 & 3759 \\
\checkmark & \checkmark &  & 3.147 & 702 & \textbf{2.180} & 3830 \\
\checkmark &  & &  \textbf{3.480} & \textbf{569}              & 2.091            & \textbf{3660} \\ \hline \hline
\multicolumn{3}{c|}{Real dataset} & \multicolumn{1}{l|}{5.66} & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{7.29} & 0.014 \\
\cline{1-7}\cline{1-7}
\end{tabular}
%\vspace{3mm}
\caption{Ablation study of self-supervision tasks. Predicting AoT improves the baseline while predicting rotation does not.}
\label{tab:ablation_temporal}
\end{table}


==> tables/ablation_temporal_renew.tex <==

\begin{table}[h]
\centering
\begin{tabular}{cccc|c|c|c|c}
\cline{1-8}\cline{1-8}
\multicolumn{4}{c|}{Methods} & \multicolumn{2}{c|}{Weizmann} & \multicolumn{2}{c}{UCFsports} \\ \hline
\multicolumn{1}{c}{Shuffle} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rotation\\(frame)\end{tabular}} &
\multicolumn{1}{c}{\begin{tabular}[c|]{@{}c@{}}Rotation\\(video)\end{tabular}} & 
\multicolumn{1}{c|}{AoT} &
\multicolumn{1}{c|}{IS($\uparrow$)} & \multicolumn{1}{c|}{FID($\downarrow$)} & \multicolumn{1}{c|}{IS($\uparrow$)} & \multicolumn{1}{c}{FID($\downarrow$)} \\ \hline
\hline
\multicolumn{4}{c|}{} & 4.264 & - & 2.749 & - \\
\checkmark &            &            &  & 4.233 & - &  & - \\
           &\checkmark  &            &  & 4.055 & - & 3.014 & - \\
           &            & \checkmark &            & 4.297 & - & 2.864 & - \\
           &\checkmark  & \checkmark &  & 4.167 & - & 2.862 & - \\
%\checkmark &           &            & \checkmark & 4.158 & - & \textbf{3.115} & - \\
%\checkmark &           & \checkmark &            & 4.313 & - & 2.930 & - \\
           &            &            &  \checkmark& \textbf{4.419} & - & \textbf{3.061} & - \\ \hline \hline
\multicolumn{4}{c|}{Real dataset} & \multicolumn{1}{l|}{5.66} & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{7.29} & 0.014 \\
\cline{1-8}\cline{1-8}
\end{tabular}
\vspace{3mm}
\caption{Ablation study of self-supervision tasks. Predicting AoT improves the baseline \kb{while predicting rotation and shuffling do not.}}
\label{tab:ablation_temporal}
\end{table}


==> tables/ablation_temporal_v2.tex <==

\begin{table}[h]
\centering
\begin{tabular}{l|c|c|c|c}
\cline{1-5}\cline{1-5}
\multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c|}{Weizmann} & \multicolumn{2}{c}{UCFsports} \\ \cline{2-5}
%\multicolumn{1}{c}{Shuffle} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rotation\\(frame)\end{tabular}} &
%\multicolumn{1}{c}{\begin{tabular}[c|]{@{}c@{}}Rotation\\(video)\end{tabular}} & 
%\multicolumn{1}{c|}{AoT} &
&\multicolumn{1}{c|}{IS($\uparrow$)} & \multicolumn{1}{c|}{FID($\downarrow$)} & \multicolumn{1}{c|}{IS($\uparrow$)} & \multicolumn{1}{c}{FID($\downarrow$)} \\ \hline
\hline
MoCoGAN(Baseline)~\cite{tulyakov2018mocogan}& 4.264 & - & 2.749 & - \\\hline
~~ + Shuffled & 4.233 & - &  & - \\
~~ + Rotation(frame) & 4.055 & - & 3.014 & - \\
~~ + Rotation(video)& 4.297 & - & 2.864 & - \\
~~ + Rotation(frame$\&$video)& 4.167 & - & 2.862 & - \\
~~ + \textbf{AoT(\textit{ours})}& \textbf{4.419} & - & \textbf{3.061} & - \\ \hline \hline
\multicolumn{1}{c|}{Real dataset} & \multicolumn{1}{l|}{5.66} & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{7.29} & 0.014 \\
\cline{1-5}\cline{1-5}
\end{tabular}
\vspace{3mm}
\caption{Ablation study of self-supervision tasks. Predicting AoT improves the baseline \kb{while predicting rotation and shuffling do not.}}
\label{tab:ablation_temporal}
\end{table}


==> tables/ablation_temporal_v3.tex <==

\begin{table}[h]
\centering
\begin{tabular}{c|l|cc|cc}
\cline{1-6}\cline{1-6}
\multicolumn{1}{c|}{\multirow{2}{*}{Baseline}}& %\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Self supervisory\\tasks\end{tabular}}} 
\multicolumn{1}{c|}{\multirow{2}{*}{Self-supervisory tasks}}
& \multicolumn{2}{c|}{\textit{Weizmann}} & \multicolumn{2}{c}{\textit{UCFsports}} \\ \cline{3-6}
%\multicolumn{1}{c}{Shuffle} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rotation\\(frame)\end{tabular}} &
%\multicolumn{1}{c}{\begin{tabular}[c|]{@{}c@{}}Rotation\\(video)\end{tabular}} & 
%\multicolumn{1}{c|}{AoT} &
& &\multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c|}{~~~FID($\downarrow$)~~~} & \multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c}{~~~FID($\downarrow$)~~~} \\ \hline
\hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}MoCoGAN\\\cite{tulyakov2018mocogan}\end{tabular}}}&~~ (a) -&~~~4.254$\pm$.01~~~& 503 &~~~2.735$\pm$.02~~~& 3828 \\
&~~ (b) Shuffled & 4.228$\pm$.01 & 527 & 2.879$\pm$.01 & 3846 \\
&~~ (c) Rotation($D_{\textit{frame}}$) & 4.043$\pm$.01 & 502 & 2.856$\pm$.01 & 4091 \\
&~~ (d) Rotation($D_{\textit{video}}$)& 4.269$\pm$.01 & 501 & 2.771$\pm$.06 & 3893 \\
&~~ (e) Rotation($D_{\textit{frame}}$$\&$$D_{\textit{video}}$)~~~& 4.186$\pm$.01 & 516 & 2.851$\pm$.02 & 3805 \\
&~~ (f) \textbf{AoT(\textit{ours})}& \textbf{4.414}$\pm$.00 & \textbf{463} & \textbf{3.098}$\pm$.01 & \textbf{3796}  \\\hline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}VGAN\\\cite{vondrick2016generating}\end{tabular}}}&~~ (a) -& 2.303$\pm$.01 & 592 & 1.224$\pm$.00 & 5160 \\
&~~ (f) \textbf{AoT(\textit{ours})}& \textbf{3.368}$\pm$.01 & \textbf{552} & \textbf{2.516}$\pm$.02 & \textbf{5026} \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}TGAN\\\cite{saito2017temporal}\end{tabular}}}&~~ (a) - & 3.584$\pm$.01 & 538 & 2.386$\pm$.02 & 3922 \\
&~~ (f) \textbf{AoT(\textit{ours})}& \textbf{4.328}$\pm$.02 & \textbf{467} & \textbf{2.802}$\pm$.02 & \textbf{3825}
\\\hline \hline
\multicolumn{2}{c|}{Real dataset} & \multicolumn{1}{c}{5.66} & \multicolumn{1}{c|}{0.008} & \multicolumn{1}{c}{7.29} & 0.014 \\
\cline{1-6}\cline{1-6}
\end{tabular}
\vspace{3mm}
\caption{Ablation study of self-supervision tasks. Predicting AoT improves the baseline \kb{while predicting rotation and shuffling do not.}}
\label{tab:ablation_temporal}
\end{table}


==> tables/ablation_temporal_v4.tex <==

\begin{table*}[width=1.0\textwidth]
\caption{Ablation study of self-supervision tasks. (a) indicates each baseline, and (b)$\sim$(f) indicates that self-supervisory tasks are adapted on (a), respectively. Predicting AoT(f) improves the baseline while verifying order(b), and predicting rotation(c-e) do not. The higher IS and the lower FVD mean better performance.}
\centering\resizebox{.97\textwidth}{!}{
\begin{tabular}{c|l|cc|cc}
\cline{1-6}\cline{1-6}
\multicolumn{1}{c|}{\multirow{2}{*}{Baseline}}& %\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Self supervisory\\tasks\end{tabular}}} 
\multicolumn{1}{c|}{\multirow{2}{*}{Self-supervisory tasks}}
& \multicolumn{2}{c|}{\textit{Weizmann}} & \multicolumn{2}{c}{\textit{UCFsports}} \\ \cline{3-6}
%\multicolumn{1}{c}{Shuffle} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rotation\\(frame)\end{tabular}} &
%\multicolumn{1}{c}{\begin{tabular}[c|]{@{}c@{}}Rotation\\(video)\end{tabular}} & 
%\multicolumn{1}{c|}{AoT} &
& &\multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c|}{~~~FVD($\downarrow$)~~~} & \multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c}{~~~FVD($\downarrow$)~~~} \\ \hline
\hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}MoCoGAN\\\cite{tulyakov2018mocogan}\end{tabular}}} &~~ (a) -~(baseline)&~~4.254$\pm$.01~~~& 31.23$\pm$.26 &~~2.735$\pm$.02~~~& 68.47$\pm$1.6\\
&~~ (b) Shuffled & 4.228$\pm$.01 & 34.57$\pm$.38 & 2.879$\pm$.01 & 70.19$\pm$1.1\\
&~~ (c) Rotation($D_{\textit{frame}}$) & 4.043$\pm$.01 & 33.03$\pm$.25 & 2.856$\pm$.01 & 75.93$\pm$.70 \\
&~~ (d) Rotation($D_{\textit{video}}$)& 4.269$\pm$.01 & 34.27$\pm$.11 & 2.771$\pm$.06 & 70.25$\pm$1.5 \\
&~~ (e) Rotation($D_{\textit{frame}}$~\&~$D_{\textit{video}}$)~~~& 4.186$\pm$.01 & 28.73$\pm$.34 & 2.851$\pm$.02 & 69.53$\pm$.92 \\
&~~ (f) \textbf{AoT(\textit{ours})}& \textbf{4.414}$\pm$.00 & \textbf{28.24}$\pm$.07 & \textbf{3.013}$\pm$.01 & \textbf{68.07}$\pm$.07  \\\hline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}VGAN\\\cite{vondrick2016generating}\end{tabular}}}&~~ (a) -~(baseline)& 2.303$\pm$.01 & 46.91$\pm$.32 & 1.224$\pm$.00 & 100.16$\pm$.71 \\
&~~ (f) \textbf{AoT(\textit{ours})}& \textbf{3.368}$\pm$.01 & \textbf{40.99}$\pm$.36 & \textbf{2.516}$\pm$.02 & \textbf{93.52}$\pm$2.5 \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}TGAN\\\cite{saito2017temporal}\end{tabular}}}&~~ (a) -~(baseline)& 3.584$\pm$.01 & 34.62$\pm$.33 & 2.386$\pm$.02 & 80.86$\pm$1.6 \\
&~~ (f) \textbf{AoT(\textit{ours})}& \textbf{4.328}$\pm$.02 & \textbf{27.89}$\pm$.17 & \textbf{2.802}$\pm$.02 & \textbf{76.91}$\pm$1.5
\\\hline \hline
\multicolumn{2}{c|}{Real dataset} & \multicolumn{1}{c}{5.636} &  \multicolumn{1}{c|}{6.02} & \multicolumn{1}{c}{6.104} & 16.55 \\
\cline{1-6}\cline{1-6}
\end{tabular}
}
\label{tab:ablation_temporal}
\end{table*}


==> tables/effectiveness_AoT_v1.tex <==

\begin{table*}[width=1.0\textwidth]
\caption{Quantitative results of ArrowGANs in video-IS. ArrowGAN framework improves all three baselines on all datasets. $\dagger$ notices that IS values are taken from MoCoGAN~\cite{tulyakov2018mocogan}, and other values are taken from our reproduced models.}
\centering\resizebox{.97\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc}
\cline{1-7}\cline{1-7}
\multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c|}{\textit{Weizmann}} & \multicolumn{2}{c|}{\textit{UCFsports}} & \multicolumn{2}{c}{\textit{UCF-101}} \\ \cline{2-7}
%\multicolumn{1}{c}{Shuffle} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rotation\\(frame)\end{tabular}} &
%\multicolumn{1}{c}{\begin{tabular}[c|]{@{}c@{}}Rotation\\(video)\end{tabular}} & 
%\multicolumn{1}{c|}{AoT} &
&\multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c|}{~~~FVD($\downarrow$)~~~} & \multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c|}{~~~FVD($\downarrow$)~~~} & \multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c}{~~~FVD($\downarrow$)~~~}\\ \hline \hline

{VGAN~\cite{vondrick2016generating}} & 2.30$\pm$.01 & 46.91$\pm$.32 & 1.22$\pm$.00 & 100.16$\pm$.71 & 8.63$\pm$.01 / 8.18$\pm.05^{\dagger}$ & 85.64$\pm$.06\\ 
{TGAN~\cite{saito2017temporal}} & 3.58$\pm$.01 & 34.62$\pm$.33 & 2.39$\pm$.02 & 80.86$\pm$1.6  & 11.17$\pm$.02 / 11.85$\pm.07^{\dagger}$ & 35.70$\pm$.13\\ 
{MoCoGAN~\cite{tulyakov2018mocogan}} & 4.25$\pm$.01 & 31.23$\pm$.26 & 2.74$\pm$.02 & 68.47$\pm$1.6  & 11.29$\pm$.07 / 12.42$\pm.03^{\dagger}$ & 36.15$\pm$.09 \\
{C*MoCoGAN~\cite{tulyakov2018mocogan}} & -$\pm$.- & -$\pm$.- & -$\pm$.- & -$\pm$-  & 12.32$\pm$.14 & 41.06$\pm$.05 \\
\hline
{Arrow-VGAN} & \textbf{3.37}$\pm$.01 & \textbf{40.99}$\pm$.36 & \textbf{2.52}$\pm$.02 & \textbf{93.25}$\pm$2.5  & \textbf{10.58}$\pm$.08 & \textbf{83.46}$\pm$.09\\ %($\uparrow1.95$)
{Arrow-TGAN} & \textbf{4.33}$\pm$.02 & \textbf{27.89}$\pm$.17 & \textbf{2.80}$\pm$.02 & \textbf{76.91}$\pm$1.5  & \textbf{12.45}$\pm$.09 & \textbf{35.16}$\pm$.05\\  %($\uparrow1.28$)
{Arrow-MoCoGAN} & \textbf{4.41}$\pm$.00 & \textbf{28.24}$\pm$.07 & \textbf{3.01}$\pm$.01 & \textbf{68.07}$\pm$.07  & \textbf{12.18}$\pm$.02 & \textbf{34.37}$\pm$.07\\ %($\uparrow0.89$)
{Arrow-C*MoCoGAN} & \textbf{-}$\pm$.- & \textbf{-}$\pm$.- & \textbf{-}$\pm$.- & \textbf{-}$\pm$.-  & \textbf{14.42}$\pm$.- & \textbf{-}$\pm$.-\\
\hline \hline
\multicolumn{1}{c|}{Real dataset} & \multicolumn{1}{c}{5.64} &  \multicolumn{1}{c|}{6.02} & \multicolumn{1}{c}{6.10} & 16.55 & \multicolumn{1}{c}{34.55} & 0.68 \\
\cline{1-7}\cline{1-7}
\end{tabular}
}
\label{tab:ablation_temporal}
\end{table*}


==> tables/effectiveness_AoT_v2.tex <==

\begin{table*}[width=1.0\textwidth]
\caption{Quantitative results of ArrowGANs in video-IS. ArrowGAN framework improves all three baselines on all datasets. $\dagger$ notices that IS values are taken from MoCoGAN~\cite{tulyakov2018mocogan}, and other values are taken from our reproduced models.}
\centering\resizebox{.97\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc}
\cline{1-8}\cline{1-8}
\multicolumn{1}{c|}{\multirow{2}{*}{Settings}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c|}{\textit{Weizmann}} & \multicolumn{2}{c|}{\textit{UCFsports}} & \multicolumn{2}{c}{\textit{UCF-101}} \\ \cline{3-7}
%\multicolumn{1}{c}{Shuffle} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rotation\\(frame)\end{tabular}} &
%\multicolumn{1}{c}{\begin{tabular}[c|]{@{}c@{}}Rotation\\(video)\end{tabular}} & 
%\multicolumn{1}{c|}{AoT} &
& &\multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c|}{~~~FVD($\downarrow$)~~~} & \multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c|}{~~~FVD($\downarrow$)~~~} & \multicolumn{1}{c}{IS($\uparrow$)} & \multicolumn{1}{c}{~~~FVD($\downarrow$)~~~}\\ \hline \hline

\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Uncond\end{tabular}}}&
{VGAN~\cite{vondrick2016generating}} & 2.30$\pm$.01 & 46.91$\pm$.32 & 1.22$\pm$.00 & 100.16$\pm$.71 & 8.63$\pm$.01 / 8.18$\pm.05^{\dagger}$ & 85.64$\pm$.06\\ 

&{TGAN~\cite{saito2017temporal}} & 3.58$\pm$.01 & 34.62$\pm$.33 & 2.39$\pm$.02 & 80.86$\pm$1.6  & 11.17$\pm$.02 / 11.85$\pm.07^{\dagger}$ & 35.70$\pm$.13\\ 
&{MoCoGAN~\cite{tulyakov2018mocogan}} & 4.25$\pm$.01 & 31.23$\pm$.26 & 2.74$\pm$.02 & 68.47$\pm$1.6  & 11.29$\pm$.07 / 12.42$\pm.03^{\dagger}$ & 36.15$\pm$.09 \\
\cline{2-8}

&{Arrow-VGAN} & \textbf{3.37}$\pm$.01 & \textbf{40.99}$\pm$.36 & \textbf{2.52}$\pm$.02 & \textbf{93.25}$\pm$2.5  & \textbf{10.58}$\pm$.08 & \textbf{83.46}$\pm$.09\\ %($\uparrow1.95$)

&{Arrow-TGAN} & \textbf{4.33}$\pm$.02 & \textbf{27.89}$\pm$.17 & \textbf{2.80}$\pm$.02 & \textbf{76.91}$\pm$1.5  & \textbf{12.45}$\pm$.09 & \textbf{35.16}$\pm$.05\\  %($\uparrow1.28$)

&{Arrow-MoCoGAN} & \textbf{4.41}$\pm$.00 & \textbf{28.24}$\pm$.07 & \textbf{3.01}$\pm$.01 & \textbf{68.07}$\pm$.07  & \textbf{12.18}$\pm$.02 & \textbf{34.37}$\pm$.07\\ %($\uparrow0.89$)
\cline{1-8}

\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\Cond\end{tabular}}}&{\begin{tabular}[c]{@{}c@{}}Categorical\\MoCoGAN~\cite{tulyakov2018mocogan}\end{tabular}} & 4.41$\pm$.01 & 30.69$\pm$.06 & 3.21$\pm$.01 & 85.88$\pm$1.3 & 12.32$\pm$.14 & 41.06$\pm$.05 \\
\cline{2-8}
&{\begin{tabular}[c]{@{}c@{}}Arrow-Categorical\\MoCoGAN\end{tabular}} & \textbf{-}$\pm$.- & \textbf{-}$\pm$.- & \textbf{-}$\pm$.- & \textbf{-}$\pm$.-  & \textbf{14.42}$\pm$.- & \textbf{-}$\pm$.-\\
\hline \hline
\multicolumn{2}{c|}{Real dataset} & \multicolumn{1}{c}{5.64} &  \multicolumn{1}{c|}{6.02} & \multicolumn{1}{c}{6.10} & 16.55 & \multicolumn{1}{c}{34.55} & 0.68 \\
\cline{1-8}\cline{1-8}
\end{tabular}
}
\label{tab:ablation_temporal}
\end{table*}


==> tables/effectiveness_of_arrowgan.tex <==
\begin{table*}[h]
\centering
\resizebox{.80\textwidth}{!}{
\smallskip\begin{tabular}{c|c|c|c}
    \cline{1-4}\cline{1-4}
     & \multicolumn{1}{c|}{\textit{UCF-101}} & \multicolumn{2}{c|}{\textit{Weizmann}}& \multicolumn{2}{c}{\textit{UCFsports}}  \\ \cline{2-6}
    Method & IS($\uparrow$)  & IS($\uparrow$) & IS($\uparrow$)\\
    \hline\hline
    {VGAN} & 9.27$\pm$.03 / 8.18 $\pm$$.05^{\dagger}$  & 2.62$\pm$.02 & 1.22$\pm$.00 \\ 
    {TGAN} & 11.17$\pm$.02 / 11.85$\pm$$.07^{\dagger}$  & 3.59$\pm$.01& 2.39$\pm$.02\\ 
    {MoCoGAN} & 10.25$\pm$.05 / 12.42$\pm$$.03^{\dagger}$ & 4.25$\pm$.01 &  2.74$\pm$.01\\  \cline{1-4}
    {Arrow-VGAN} & 10.47$\pm$.14 & 3.33$\pm$.01 &  2.49$\pm$.01  \\
    {Arrow-TGAN} & 12.51$\pm$.06 & 4.32$\pm$.02 &  2.81$\pm$.23  \\
    {Arrow-MoCoGAN} & 11.18$\pm$.03  & 4.41$\pm$.01 & 2.76$\pm$.01 \\
    \cline{1-4}
    {Real dataset} & 34.49 & 5.66 & 7.29\\
    \cline{1-4}\cline{1-4}
  \end{tabular}
}
\vspace{3mm}
\caption{Effectiveness of adding ArrowGAN on baselines. It improves all three baselines in UCF-101. $\dagger$ notices that IS values are taken from MoCoGAN~\cite{tulyakov2018mocogan}, and other values are taken from our reproduced models.}
\label{tab:Uncond UCF101}
\end{table*}

==> tables/effectiveness_of_arrowgan_IS.tex <==
\begin{table*}[h]
\centering
\resizebox{.80\textwidth}{!}{
\smallskip\begin{tabular}{c|c|c|c}
    \cline{1-4}\cline{1-4}
     & \multicolumn{1}{c|}{\textit{UCF-101}} & \multicolumn{2}{c|}{\textit{Weizmann}}& \multicolumn{2}{c}{\textit{UCFsports}}  \\ \cline{2-6}
    Method & IS($\uparrow$)  & IS($\uparrow$) & IS($\uparrow$)\\
    \hline\hline
    {VGAN} & 9.27$\pm$.03 / 8.18 $\pm$$.05^{\dagger}$  & 2.62$\pm$.02 & 1.22$\pm$.00 \\ 
    {TGAN} & 11.17$\pm$.02 / 11.85$\pm$$.07^{\dagger}$  & 3.59$\pm$.01& 2.39$\pm$.02\\ 
    {MoCoGAN} & 10.25$\pm$.05 / 12.42$\pm$$.03^{\dagger}$ & 4.25$\pm$.01 &  2.74$\pm$.01\\  \cline{1-4}
    {Arrow-VGAN} & 10.47$\pm$.14 & 3.33$\pm$.01 &  2.49$\pm$.01  \\
    {Arrow-TGAN} & 12.51$\pm$.06 & 4.32$\pm$.02 &  2.81$\pm$.23  \\
    {Arrow-MoCoGAN} & 11.18$\pm$.03  & 4.41$\pm$.01 & 2.76$\pm$.01 \\
    \cline{1-4}
    {Real dataset} & 34.49 & 5.66 & 7.29\\
    \cline{1-4}\cline{1-4}
  \end{tabular}
}
\vspace{3mm}
\caption{Effectiveness of adding ArrowGAN on baselines. It improves all three baselines in UCF-101. $\dagger$ notices that IS values are taken from MoCoGAN~\cite{tulyakov2018mocogan}, and other values are taken from our reproduced models.}
\label{tab:Uncond UCF101}
\end{table*}
